Predicting Question-Answering Performance of Large Language Models through Semantic Consistency

Semantic consistency of a language model is broadly defined as the model's ability to produce semantically-equivalent outputs, given semantically-equivalent inputs. We address the task of assessing question-answering (QA) semantic consistency of contemporary large language models (LLMs) by manually creating a benchmark dataset with high-quality paraphrases for factual questions, and release the dataset to the community. We further combine the semantic consistency metric with additional measurements suggested in prior work as correlating with LLM QA accuracy, for building and evaluating a framework for factual QA reference-less performance prediction -- predicting the likelihood of a language model to accurately answer a question. Evaluating the framework on five contemporary LLMs, we demonstrate encouraging, significantly outperforming baselines, results.

==> chapters/5-qa-prediction-regression-analysis.back.tex <==
\section{QA Performance Prediction}
\label{sec:performance-prediction}

%\ella{justify predictors -- distinct works independently developed the hypothesis that question entity popularity, uncertainty and consistency (mainly this work) affect a model's ability to answer a question correctly; we consolidate the hypotheses, reproduce findings on the same dataset and test the predictive power of these factors on the dependent variable}

We next define and address the task of factoid question-answering performance prediction. Factoid question typically call for a single correct answer that consists of one or a small number of words that constitute the precise answer to the question. Here we rely on some parallels to Query performance prediction (QPP) in IR systems -- an established field of research \ella{references}. QPP is defined as the assessment of the retrieval quality of a search system for a query without relevance judgments. However, there also exist core differences between IR (search) systems and LLM-based architectures used for the task of open-domain factoid QA; yet, we address a conceptually similar task: assessment of a system's potential answer quality (that is manifested by its correctness) for a question, without relying on reference answers.

Casting the question as a classification task, we train a logistic regression model, where several predictors---variables proven to correlate with model's accuracy---carry over predictive power on the outcome variable: the model's likelihood to produce a correct answer for a given question.  

\subsection{Predictor Variables}

Here, we attempt to predict correctness of original questions $q\in\textrm{PopQA}$ \texrm{only} by leveraging 
additional information obtained from their paraphrases $P(q)$ in PopQA-TP.  Thus all predictor variables are associated with $q$.

\subsubsection{Question Subject Popularity (SPop)
\label{ssec:subject_popularity}}
\citet{mallen2023not} hypothesize that factual knowledge that is less frequently discussed on the web may not be well memorized by LLMs. Given a question that can be modeled by the \{subject, relationship, object\} triple, e.g., "What is the \textit{capital of} (R) \textit{Louisiana} (S)?", the authors approximate its subject's popularity by the mean number of monthly views of the corresponding Wikipedia page. The answer---"Baton Rouge"---is scored by popularity in a similar way, but we refrain from using this score for our predictive analysis, since it's unknown in a realistic QA setup.

Following \citet{mallen2023not}, we define our first predictor---question subject popularity (SPop)---as the mean number of monthly views of the subject entity's Wikipedia page. In the PopQA dataset, SPop score varies from 2 to over 15M.

\subsubsection{Semantic Consistency (SCons)}
\label{sec:semantic-consistency-predictor}

The semantic consistency---as defined by the SCOns metric in Section~\ref{ssec:consistency-metrics}---associated with $q$ is measured as $\textrm{SCons}(\mathcal{A})$, where $\mathcal{A}$ consists of the answers to $q$ itself and its paraphrases $P(q)$.


%Following the definition of the semantic consistency metric in Section~\ref{ssec:consistency-metrics}, we compute the semantic consistency of a set of sampled answers $\mathcal{A}$ to a factoid question $q\in\textrm{PopQA}$, as the mean pairwise cosine similarity of the answers' encodings.


\subsubsection{Semantic Certainty (SCert)}
\label{sec:semantic-certainty}
Multiple studies investigated the \textit{uncertainty} of natural language generation in the context of free-form QA. \ella{references from kuhn et al.} In their recent work, \citet{kuhn2022semantic} put forward a hypothesis that given some degree of freedom (i.e., sampling, not greedy generation), ``$\dots$very \textit{uncertain} generations should be less likely to be \textit{correct}". Practically, the authors suggest that a (non-greedily-probed) model producing multiple distinct answers for the same question is unstable and less robust, potentially affecting the model's ability to provide a correct answer to the question.

Uncertainty of a set of answers $\mathcal{A}$ to a factoid question $\mathcal{Q}$ is manifested by the relative amount of distinct answers out of the entire answer pool $\mathcal{A}$. Multiple metrics were suggested to measure uncertainty---or, its complementary metric, \textit{certainty}---of a set of answers, including lexical similarity, Rouge-L \cite{lin2004rouge}, and predictive entropy \citep{kuhn2022semantic}. As with semantic consistency (see Section~\ref{sec:semantic-consistency-predictor}), we found mean pairwise semantic similarity of answers in $\mathcal{A}$ to be the most appropriate metric for certainty of very short factoid answers. Table ... presents several results of sampling answers to questions in the PopQA dataset, along with their respective certainty score. The score is computed by mean pairwise cosine similarity of the set of answer representations (embeddings), extracted using the SentenceTransformers package\footnote{https://www.sbert.net/} \citep{reimers-2019-sentence-bert}.

\begin{table*}[hbt]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|l|c}
question & sampled answers & certainty score \\ \hline
What is Robby Krieger’s occupation? & (guitarist, guitarist, guitarist, guitarist, guitarist) & 1.000 \\
What is Shozaburo Nakamura's occupation? & (samurai, samurai, film director, actor, director) & 0.250 \\
more examples & ... & ... \\

\end{tabular}
}
\caption{Examples of certainty score assigned to a set of answers to the same question. \ella{can say something about the inherent cultural bias manifested by the samurai answer...}}
\label{tbl:certainty-scores}
\end{table*}

We, therefore, define our next predictor -- sampled answers certainty (SCert) -- as the mean pairwise cosine similarity of the set of answer embeddings. Naturally, SCert varies between 0 and 1.

\subsubsection{Question Category (QCat)}
\label{ssec:question_category}
Figure~\ref{fig:models-correctness} suggests that question category---the semantic grouping a question belongs to---has a considerable effect on a model's ability to answer a question correctly. While models systematically succeed in answering questions on \textit{capital}, \textit{color}, and \textit{sport}, they struggle in categories like \textit{director}, \textit{producer}, and \textit{author}. Figure ... provides further evidence for the effect of question category on QA correctness, suggestive of the potential benefits of including question category as a (nominal) categorical variable in regression analysis.


\subsection{Predictive Model}

%\ella{logistic regression model description from the next section; results will be left to the next section}

We propose to build a statistical model to predict if a generative model will answer a given question correctly.  The question considered is an original PopQA question $q$, where we consider additional information from the paraphrases $P(q)$ (see Section~\ref{ssec:manual_paraphrases}) we form.  For a given $q$, define variables:

\begin{itemize}
\item \textbf{CORRECT} (binary): 1 if $q$ was answered correctly by the model, otherwise 0
\item \textbf{CATEGORY}: question $q$ category label
\item \textbf{CONS\_COS}: semantic consistency of answers to  $P(q)$  (Section~\ref{sec:semantic-consistency-predictor})
\item \textbf{CERT\_COS}: semantic certainty among answers repeatedly sampled to question $q$  (Section~\ref{sec:semantic-certainty}).
\item \textbf{LOG\_S\_POP}: natural log of the popularity of $q$'s subject (following the definition in \citealp{mallen2023not}, detailed in Section~\ref{ssec:subject_popularity})
\end{itemize}

\noindent
The numeric values of CONS\_COS, CERT\_COS, and LOG\_S\_POP are standardized within given results of PopQA\_TP for a given LLM before input into the predictive model.  Figure~\ref{fig:std_variable_kde_grouped} shows kernel density estimates (KDEs) of the resulting variable distributions by CATEGORY value.

\begin{figure}[h!]
\centering
\includegraphics[width=0.49\textwidth]{semantic_consistency/figures/google_flan_ul2_bygroup_kdeplot_std.png}
\caption{KDE of standardized values of dataset numeric variables, by question CATEGORY value. 
 There is significant variation in the variable ranges, including the popularity, between categories.}
\label{fig:std_variable_kde_grouped}
\end{figure}

We use a logistic regression model to predict the binary outcome CORRECT$\in\{0,1\}$.  Logistic regression models the unobserved probability that CORRECT=1, which we denote by the variable PCORRECT$\in[0,1]$, and taking its logit (log odds) transformation.  The logit of PCORRECT is modeled as a linear additive function a set of regressor variables, typically consisting of a set of predictor variables with possible interactions between them.  The model assumes a linear relationship between each regressor and the logit of the binary target, holding other regressors constant.  Logistic regression is performed using Python's \texttt{statsmodels} \citep{seabold2010statsmodels} module formula interface. 

Our predictive model is specified as $LOGIT(PCORRECT)\:\sim\: (CATEGORY * LOG\_S\_POP)\: + \:(CATEGORY * CONS\_COS) + \:(CATEGORY * CERT\_COS)$.
That is, we consider the first-order effects of the standardized numeric variables (LOG\_S\_POP, CONS\_COS, and CERT\_COS) and CATEGORY, as well as the second-order interaction between each numeric variable (but not each other) and CATEGORY.  CATEGORY is treated as a fixed rather than random categorical effect, since we are interested in the individual effect of each category and do not assume that the relationship types were randomly sampled from the population of available ones.  

In the following, we will use the results of the flan-ul2 model, which has approximately 12.5\% correctness on our dataset PopQA\_TP. 

For the following figures, we discretize the observed ranges of the standardized numeric variables into equal-length bins, and calculate the empirical average of the values of the CORRECT variable (which we call ECORRECT) for variable values in each bin; this approximates the typical value of PCORRECT, which is unobserved, within each bin.  The logit of ECORRECT is plotted vs the binned variable values to assess the relationship's linearity, which impacts the appropriateness of the logistic model.

Figure~\ref{fig:logit_correctness_vs_single_vars} shows the logit of ECORRECT for each numeric variable overall (left) and by each level of CATEGORY, within the fixed bins.  In the left plot, the vertical red lines contain the middle 95\% of un-binned variable values; on either side, there tend to be relatively few observations given the interval width, and any such observations may be outliers.  Thus we see that the CONS\_COS and CERT\_COS measures have a roughly linear relationship with the logit, particularly within the middle 95\% interval, which supports the addition of the individual variables; LOG\_S\_POP is more unusual, having a bimodal relationship.  In the right plot, the logit is plotted vs the variable only within this 95\% interval, for each level of CATEGORY.  In many cases, a roughly linear relationship still holds, which justifies the regression on the CATEGORY factor; this is manifested in the line plots having different vertical displacement, but the same slopes for different categories.  Furthermore, the slopes of some lines differ, which is evidence of an interaction between CATEGORY and the variable.  This is particularly true of the LOG\_S\_POP variable, which is reflected in Table~\ref{tbl:predictor-logistic-regression}, where the CATEGORY interactions for LOG\_S\_POP tend to be more significant than for other two variables.


\begin{figure*}[h!]
\centering
\includegraphics[width=0.49\textwidth]{semantic_consistency/figures/google_flan_ul2_logit_pcorrect_lineplot.png}
\includegraphics[width=0.49\textwidth]{semantic_consistency/figures/google_flan_ul2_bygroup_logit_pcorrect_lineplot.png}
\caption{Left: Logit of average correctness within equal-length bins of LOG\_S\_POP (left), CONS\_COS (middle), and CERT\_COS (right).  The dashed vertical lines indicate the range of the variables' quantiles 0.025 and 0.975, the middle 95\% interval.\\
Right: The same line plots, conditioned on levels of the CATEGORY variable.}
\label{fig:logit_correctness_vs_single_vars}
\end{figure*}

For each regressor variable, its associated odds ratio $r$ is calculated as $r=e^{\hat{\beta}}$, where $\hat{\beta}$ is the estimated regressor coefficient.  Table~\ref{tbl:predictor-logistic-regression} shows the estimated odds ratios and their 95\% confidence intervals.  The interpretation of an odds ratio value $r$ is the multiplicative change in $\textrm{PCORRECT}/(1-\textrm{PCORRECT})$ associated with a 1-unit change in the regressor.  For the numeric variables, which have been standardized, this corresponds to a 1 standard deviation change (allowing their effect to be compared despite the different original scales); for the factor CATEGORY, this corresponds to the increase in the odds ratio associated with the given category value relative to that of the omitted level, `author'.  Here, $r>1$ ($\hat{\beta}>0$) indicates a positive correlation between the regressor and the likelihood of a correct prediction.  The regressor is statistically significant if its odds ratio differs significantly from 1 in either direction, as indicated by the confidence interval.


%\ella{we should have a heatmap of pairwise predictor correlations, regression analysis}


==> chapters/7-ethical-considerations.tex <==
\section{Ethical Considerations}
\label{sec:ethical}

\ella{not sure we need this section...}

